Taming Tail Latency for Erasure-coded, Distributed Storage Systems

Distributed storage systems are known to be susceptible to long tails in response time. In modern online storage systems such as Bing, Facebook, and Amazon, the long tails of the service latency are of particular concern. with 99.9th percentile response times being orders of magnitude worse than the mean. As erasure codes emerge as a popular technique to achieve high data reliability in distributed storage while attaining space efficiency, taming tail latency still remains an open problem due to the lack of mathematical models for analyzing such systems. To this end, we propose a framework for quantifying and optimizing tail latency in erasure-coded storage systems. In particular, we derive upper bounds on tail latency in closed form for arbitrary service time distribution and heterogeneous files. Based on the model, we formulate an optimization problem to jointly minimize the weighted latency tail probability of all files over the placement of files on the servers, and the choice of servers to access the requested files. The non-convex problem is solved using an efficient, alternating optimization algorithm. Numerical results show significant reduction of tail latency for erasure-coded storage systems with a realistic workload.

==> beck.tex <==
\section{Proof that Alternating Minimization Converges to Optimal Solution}


The authors of \cite{1137/13094829X} showed that if the following five assumptions are satisfied for the  minimization problem
\begin{equation}
min_{{\mathbf y}\in\mathbb R^{n_1},{\mathbf z}\in\mathbb R^{n_2}}  H({\mathbf y},{\mathbf z})\equiv f({\mathbf y},{\mathbf z})+g_1({\mathbf y})+g_2({\mathbf z}) ,\label{beckmain}
\end{equation}
the alternating minimization over ${\mathbf y}$ and ${\mathbf z}$ converges to optimal solution with a sublinear rate of convergence. 

\begin{description}
\item[A]The functions $g_1:\mathbb R^{n_1} \to (-\infty,\infty]$ and $g_2:\mathbb R^{n_2} \to (-\infty,\infty]$ are closed and proper convex functions assumed to be sub-differentiable over their domain.\\
\item[B]The function $f$ is a continuously differentiable convex function over dom $g_1 \times$ dom $g_2$\\
\item[C]The gradient of $f$ is (uniformly) Lipschitz continuous with respect to the variables vector ${\mathbf y}$ over dom $g_1$ with constant $L_1 \in(0,\infty)$: $$
\Arrowvert  \nabla_1f({\mathbf y}+{\bf d_1},{\mathbf z}) -\nabla_1f({\mathbf y},{\mathbf z})\Arrowvert \le L_1 \Arrowvert {\bf d_1}\Arrowvert$$
for any ${\mathbf y} \in \text{ dom } g_1$, ${\mathbf z}\in \text{ dom } g_2$, and ${\bf d_1}\in\mathbb R^{n_1}$ such that ${\mathbf y}+{\bf d_1} \in \text{ dom } g_1$.\\
\item[D]The gradient of $f$ is Lipschitz continuous with respect to the variables vector ${\mathbf z}$ over dom $g_2$ with constant $L_2 \in(0,\infty]$: $$\Arrowvert  {\nabla_2f({\mathbf y},{\mathbf z}+{\mathbf d}_2) -\nabla_2f({\mathbf y},{\mathbf z})}\Arrowvert \le L_2 \Arrowvert {{\mathbf d}_2}\Arrowvert$$
for any ${\mathbf y} \in \text{ dom }g_1$, ${\mathbf z}\in \text{ dom } g_2$, and ${\mathbf d}_2\in\mathbb R^{n_2}$ such that ${\mathbf y}+{\mathbf d}_2 \in \text{ dom } g_2$.\\
\item[E]The optimal set of \eqref{beckmain}, denoted by $X^*$, is nonempty, and the corresponding optimal value is denoted by $H^*$. In addition, for any $\tilde{\mathbf y}\in \text{ dom } g_1$ and $\tilde{\mathbf z}\in \text{ dom } g_2$, the problems $\min_{{\mathbf z}\in\mathbb R^{n_2}} f(\tilde{\mathbf y},{\mathbf z})+g_2({\mathbf z}),$ and  $min_{{\mathbf y}\in\mathbb R^{n_1}}f(y,\tilde{z})+g_1({\mathbf y})$ have minimizers.
\end{description}\par
%If all the 5 assumptions above are proven to be true, Alternating-Minimization method can be applied for the objective minimization problem.\\ \par
\begin{tabular}{|p{9cm}|}
\hline
\textbf{The Steps of Alternating Minimization Method}\\ \\
\textbf{Step 1:} Initialization \\ ${\mathbf y}_0 \in$ dom $g_1$, ${\mathbf z}_0 \in$ dom $g_2$ such that ${\mathbf z}_0 \in \argmin_{{\mathbf z} \in \mathbb R^{n_2}}f({\mathbf y}_0,{\mathbf z})+g_2({\mathbf z})$.\\
\textbf{Step 2:} General Step (k=0,1,...)\\
$${\mathbf y}_{k+1} \in \argmin_{{\mathbf y}\in \mathbb R^{n_1}}f({\mathbf y},{\mathbf z}_k)+g_1({\mathbf y}),$$
$${\mathbf z}_{k+1} \in \argmin_{{\mathbf z}\in \mathbb R^{n_2}}f({\mathbf y}_{k+1},{\mathbf z})+g_2({\mathbf z})$$
\textbf{Step 3:} Decide the optimal set\\
The k-th iterate will be denoted by $\vec x_k=({\mathbf y}_k.{\mathbf z}_k)$, the generated sequence is monotone and satisfies:$$H(\vec x_0)\ge H(\vec x_1)\ge H(\vec x_2)\ge H(\vec x_3)\ge \ldots$$When $H(\vec x_{k+1})-H(\vec x_k) \to 0$ ,decide this $\vec x_k$ is the optimal arg.\\
\hline
\label{amintabl}
\end{tabular}\\ \\
%\begin{proof}


 In order to prove optimality of alternating minimization for our problem, we first transfer the constraints of our problem into the objective function. In order to do that, let
\begin{displaymath}
I(x)=\left\{ \begin{array}{ll}
0 & \textrm{if $x\ge 0$}\\
\infty & \textrm{if $x < 0$}
\end{array}\right.
\end{displaymath}\\

The problem in \eqref{objeq}-\eqref{forml} reduces to
\begin{eqnarray}
\min_{{\mathbf t},{\mathbf \pi}}&& \sum_i \omega_i \left( \sum_{j}\frac{\pi_{ij}}{e^{t_j x}} \frac{(1-\rho_j)t_j M_j(t_j)}{t_j - \Lambda_j (M_j(t_j)-1)}\right)
\nonumber\\
& &+\sum_j{I(t_j)}+\sum_j{I(-t_j(t_j-\alpha_j+\Lambda_j)-\Lambda_j\alpha_j(e^{\beta_j t_j}-1))}
\nonumber\\
 & &+\sum_i{I(K_i-\sum_j \pi_{ij})}+\sum_i{I(\sum_j \pi_{ij}-K_i)}\nonumber\\
 & &+\sum_i{\sum_j{I(\pi_{ij})}}+\sum_i{\sum_j{I(1-\pi_{ij})}}
\end{eqnarray}\\

We will now verify that the above five assumptions are satisfied for our problem.  

\begin{description}
\item[A] The function\begin{displaymath}
I(x)=\left\{ \begin{array}{ll}
0 & \textrm{if $x\ge 0$}\\
\infty & \textrm{if $x < 0$}
\end{array}\right.
\end{displaymath}
 is convex over $\mathbb R$. The functions $g_1$, $g_2$  are 
\begin{eqnarray}
&&g_1( {\bf t})\nonumber\\
&=&\sum_j{I(-t_j(t_j-\alpha_j+\Lambda_j)-\Lambda_j\alpha_j(e^{\beta_j t_j}-1))}\nonumber\\
&&+\sum_j{I(t_j)}\\
&&g_2({\bf \pi})\nonumber\\
&=&\sum_i{I(K_i-\sum_j \pi_{ij})}+\sum_i{I(\sum_j \pi_{ij}-K_i)}\nonumber\\
&&+\sum_i{\sum_j{I(\pi_{ij})}}+\sum_i{\sum_j{I(1-\pi_{ij})}}
\end{eqnarray}
The corresponding functions $g_1:\mathbb R^{n_1} \to [0,\infty]$ and $g_2:\mathbb R^{n_2} \to [0,\infty]$ h are closed and proper convex functions,  subdifferentiable over their domain. The assumption A is thus satisfied.\\
\item[B] The function $f$  is $f({\bf t},{\bf \pi})=\sum_i \omega_i \left( \sum_{j}\frac{\pi_{ij}}{e^{t_j x}} \frac{(1-\rho_j)t_j M_j(t_j)}{t_j - \Lambda_j (M_j(t_j)-1)}\right)$, it has been proven convex over $t_j$ in Theorem 3 and convex over $\pi_{ij}$ in Theorem 4. So the function $f$ is a continuously differentiable convex function over dom $g_1 \times $ dom $g_2$. The assumption B is thus satisfied.\\
\item[C] The function $f({\bf t} ,{\bf \pi})$ is differentiable w.r.t. each $t_j$ and the deriavative is bounded for 

For the function $f({\bf t} ,{\bf \pi})$, denote $A=\alpha_j\Lambda_j$, $C=\alpha_j-\Lambda_j$,
\begin{eqnarray}
\Arrowvert  \nabla_1f({\bf t}+{\bf d_1},{\bf \pi}) -\nabla_1f({\bf t},{\bf \pi})\Arrowvert =\nonumber\\ \sum_i \omega_i \sum_j\pi_{ij}\alpha e^{(\beta_j-x)t_j} M(d_{1j})\nonumber
\end{eqnarray}
\begin{eqnarray}
&&M(d_{1j})\nonumber\\
&=&\frac{t_j e^{(\beta_j-x)d_{1j}}}{X(t_{1j}+d_{1j})}-\frac{t_j}{X(t_j)}+\frac{e^{(\beta_j-x)d_{1j} }}{X(t_j+d_{1j})}d_{1j} \nonumber\\
&\le&\frac{t_j}{X(t_j+d_{1j})}-\frac{t_j}{X(t_j)}+\frac{1}{X(t_j+d_{1j})}d_{1j} \nonumber\\
&=&\frac{A e^{\beta_j t_j}(e^{\beta_j d_{1j}}-1)}{X(t_j+d_{1j})X(t_j)} +\frac{1}{X(t_j+d_{1j})}d_{1j}\nonumber\\
&&+\frac{d_{1j}+2t_j-C}{X(t_j+d_{1j})X(t_j)}d_{1j}\nonumber\\
&=&\frac{A e^{\beta_j t_j}(\sum_{i=1}\frac{\beta_j^{i+1}d_{1j}^i}{(i+1)!})}{X(t_j+d_{1j})X(t_j)}d_{1j}+\frac{1}{X(t_j+d_{1j})}d_{1j}\nonumber\\
&&+\frac{d_{1j}+2t_j-C}{X(t_j+d_{1j})X(t_j)}d_{1j}\nonumber\\
&\le& L_{1j} d_{1j}\nonumber
\end{eqnarray}
$$\Arrowvert  \nabla_1f({\bf t}+{\bf d_1},{\bf \pi}) -\nabla_1f({\bf t},{\bf \pi})\Arrowvert \le L_1 \Arrowvert {\bf d_1}\Arrowvert $$
Since $L_1 \in (0,\infty)$, The assumption C is also satisfied.\\
\item[D]For the function $f({\bf t}_j,{\bf \pi})$, denote $B=e^{-t_jx}M_j(t_j)$, $C_1 = \frac{1}{\alpha_j}+\beta_j$, $C_2 = \frac{M_j(t_j)-1}{t_j}$,
\begin{eqnarray}
\Arrowvert  \nabla_2f({\bf t},{\bf \pi}+{\mathbf d}_2) -\nabla_2f({\bf t},{\bf \pi})\Arrowvert =\nonumber\\ \sum_i \omega_i \sum_j B N(d_{2,ij})\nonumber
\end{eqnarray}
\begin{eqnarray}
&&N(d_{2,ij})\nonumber\\
&=&\pi_{ij}\left[\frac{1-\Lambda_jC_1-\lambda_id_{2,ij}C_1}{1-\Lambda_jC_2-\lambda_id_{2,ij}C_2}-\frac{1-\Lambda_jC_1}{1-\Lambda_jC_2}\right]\nonumber\\
&&+\frac{1-\Lambda_jC_1}{1-\Lambda_jC_2}d_{2,ij}\nonumber\\
&=&\frac{\pi_{ij}\lambda_i(C_2-C_1)}{(1-\Lambda_jC_2)(1-\Lambda_jC_2-\lambda_id_{2,ij}C_2)}d_{2,ij}\nonumber\\
&&+\frac{1-\Lambda_jC_1}{1-\Lambda_jC_2}d_{2,ij}\nonumber\\
&\le& L_{2,ij} d_{2,ij}\nonumber
\end{eqnarray}
$$\Arrowvert  \nabla_2f({\bf t},{\bf \pi}+{\mathbf d}_2) -\nabla_1f({\bf t},{\bf \pi})\Arrowvert \le L_2 \Arrowvert {\mathbf d}_2\Arrowvert $$
Since $L_2 \in (0,\infty]$, the assumption D is satisfied.\\
\item[E]The optimal set of \eqref{beckmain}, denoted by $X^*$ is obviously nonempty as there always exist ${\bf \pi}$ and ${\bf t}_j$ as the iteration goes.\\
\end{description}
%\end{proof} 


==> implement_old.tex <==
\section{Numerical Results}

To validate the proposed tail latency bound and tail latency optimization, we simulate erasure-coded storage systems %with chunk service time distributions from Tahoe experiments \cite{Yu_TON} and Amazon S3 experiments \cite{CS14}. We
and compare the performance of our proposed latency optimization, denoted as  WLTP Policy, with five naive strategies:

\begin{itemize}
\item Proposed Approach-Optimized Placement, i.e., WLTP-OP ({\em Weighted  Latency Tail Probability-Optimized Placement}) Policy: The joint scheduler is determined by the proposed solution that minimizes the weighted  latency tail probabilities, with respect to our proposed tail latency bounds and placement optimization. We consider optimizing the placement of the chunks of the files in this policy.

\item Proposed Approach-Random Placement, i.e., WLTP-OP ({\em Weighted  Latency Tail Probability-Random Placement}) Policy: The joint scheduler is determined by the proposed solution that minimizes the weighted  latency tail probabilities, with respect to our proposed tail latency bounds and placement optimization. The chunks are allocated randomly in this policy. 


\item PEAP-RP Policy ({\em Projected, Equal Access-Probability-Random Placement}): For each file request, the joint request scheduler selects available chunks and nodes with equal probability. The equal access-probabilities are projected toward feasible region in (\ref{objeq}) for all $t_j = .01$ to ensure stability of the storage system and the objective is then optimized over ${\mathbf t}$. We assume that the chunks of the files are randomly placed among the storage nodes. 



\item PEAP-OP Policy: This strategy is same as  PEAP-RP except that we further perform placement optimization besides optimizing scheduling probabilities $\boldsymbol{\pi}$ and auxiliary variables  $\boldsymbol{t}$.

\item  PPF-RP Policy  ({\em Projected-Proportional Fairness-Random Placement Policy}): The joint request scheduler is optimized to balance the workload (arrival rates) of all storage nodes as will be described later. Intuitively, this policy minimizes the chance of congested bottleneck in the storage system. The strategy is further optimized over ${\mathbf t}$.




\item  PPF-OP Policy  ({\em Projected-Proportional Fairness-Optimized Placement Policy}): The joint request scheduler is optimized to balance the workload (arrival rates) of all storage nodes as will be described later. Intuitively, this policy minimizes the chance of congested bottleneck in the storage system. The objective is further optimized over ${\mathbf t}$. The strategy here utilizes all $\boldsymbol{\pi}$, $\boldsymbol{t}$ and $\boldsymbol{\mathcal{S}}$ as mentioned above. Then, alternating optimization over placement and 
$\boldsymbol{t}$ are performed using the
proposed policy.





\end{itemize}

In the simulations, we consider $r=1000$ files, all of size 200 MB and using $(7,4)$ erasure code in a distributed storage system consisting of $m=12$ distributed nodes. Based on \cite{Yu_TON,CS14,Yu-TON16}, we consider chunk service time that follows a shifted-exponential distribution with rate $\alpha_j$ and shift $\beta_j$. As shown in Table~\ref{tb}, we have 12 heterogeneous storage nodes with different service speed and round-trip-time. The base arrival rates for the first 250 files is $2/150$ s$^{-1}$, for the next 250 files are $4/150$ s$^{-1}$,  for the next 250 files are $6/150$ s$^{-1}$, and for the last 250 files is $3/150$ s$^{-1}$. The first 250 files are placed on first seven nodes, the next 250 files are placed on nodes 2 to 8, the next 250 files are placed on nodes 4 to 10, and the last 250 files are placed on nodes 6 to 12. This paper also considers the weights of the files proportional to the arrival rates.  %and are thu - where the weights corresponding to the first 250 files are each chosen as $2/(15\times 250)$, the weights corresponding to the next 250 files are chosen as $4/(15\times 250)$, the weights corresponding to the next 250 files are chosen as $6/(15\times 250)$, and the weights corresponding to the last 250 files are chosen as $3/(15\times 250)$ such that the sum of weights of all files is $1$. 
 In order to initialize the algorithm, we choose $\pi_{ij} = k/n$ on the placed servers, all $t_j = .01$. However, since these choices of $\mathbf \pi$ and ${\mathbf t}$ may not be feasible, we modify the initialization ${\bm \pi}$ to be the closest norm feasible solution to the above choice.

\begin{table}[ht]
\caption{Summary of parameters for the 12 storage nodes in our simulation (shift $\beta$ in ms and rate $\alpha$ in 1/s).}\centering
  \resizebox{.48 \textwidth}{!}{
\begin{tabular}{c c c c c c c}
\hline\hline
 & Node 1 & Node 2 & Node 3  & Node 4 & Node 5 & Node 6 \\ [0.25ex]
\hline
$\alpha_j$ & 20.0015  & 26.1252 &  14.9850 & 17.0526  & 27.1422  & 22.8919 \\
$\beta_j$ & 10.5368  & 15.6018 &  8.2756  &  10.0120 &  12.8544 & 13.6722 \\ [1ex]
\hline\hline
 & Node 7 & Node 8 & Node 9  & Node 10 & Node 11 & Node 12 \\ [0.25ex]
\hline
$\alpha_j$ & 30.0000 &  21.3812  &  11.9106 & 25.1599  & 28.8188 & 23.8067  \\
$\beta_j$ & 12.6616   & 9.9156  & 10.7872 & 8.6166  & 13.8721 &  10.8964 \\ [0.25ex]
\hline
\end{tabular}}
\label{tb}
\end{table}

%The $\beta_j$ for different nodes are chosen as 8.5368 ms,   13.6018 ms,    6.2756  ms,  9.5100 ms,   9.0524 ms,  12.1242 ms,  12.3616   ms, 7.4950  ms,  9.9182 ms, 9.5646  ms, 11.1706 ms, and  11.6750 ms respectively. The $\alpha_j$ for different nodes are chosen as 18.2295  s$^{-1}$, 24.0552 s$^{-1}$,   11.8750 s$^{-1}$,  17.0526  s$^{-1}$, 26.1912  s$^{-1}$, 23.9059 s$^{-1}$,  27.0006 s$^{-1}$,  21.3812  s$^{-1}$,  9.9106 s$^{-1}$, 24.9589  s$^{-1}$, 26.5288 s$^{-1}$, and  21.8067 s$^{-1}$ respectively.


%The base arrival rates for the first 500 files are chosen as $0.02$ s$^{-1}$, for the next 5000 files is chosen as $0.03$ s$^{-1}$. The first 250 files are placed on first seven nodes, the next 250 files are placed on nodes 2 to 8, the next 250 files are placed on nodes 4 to 10, and the last 250 files are placed on nodes 6 to 12. This paper also considers different weights of the files - where the weights corresponding to the first 250 files are each chosen as $2/(15\times 250)$, the weights corresponding to the next 250 files are chosen as $4/(15\times 250)$, the weights corresponding to the next 250 files are chosen as $6/(15\times 250)$, and the weights corresponding to the last 250 files are chosen as $3/(15\times 250)$ such that the sum of weights of all files is $1$.  In order to initialize the algorithm, we choose $\pi_{ij} = k/n$ on the placed servers, all $t_j = .01$. However, since these choices of $\mathbf \pi$ and ${\mathbf t}$ may not be feasible, we modify the initialization ${\bm \pi}$ to be the closest norm feasible solution to the above choice.

\begin{figure}
	\begin{center}
		\includegraphics[trim=.0in 0in 5.7in .0in, clip,width=0.45\textwidth]{tailProb_vs_x}
		\caption{Weighted  Latency Tail Probability vs $x$ (in seconds).}
		\label{tailfig}
	\end{center}
\end{figure}




\noindent {\bf Weighted  Latency Tail Probabilities: } In Figure~\ref{tailfig}, we plot the decay of weighted  latency tail probability $\sum_i \omega_i\Pr(L_i \ge x)$ with $x$ (in seconds) for Policies WLTP, PEAP and BNW. Policy WLTP solves the optimal weighted latency tail probability via proposed alternative optimization algorithm over $t_j$ and $\pi_{i,j}$. With fixed ${\mathbf t}$, Policy PEAP uses equal server access probabilities, projected toward the feasible region, while Policy BNW load-balances chunk requests across different servers. The values of ${\mathbf t}$ are then found optimally for the above given values of $\pi_{i,j}$.   In particular, for PPF, we set the access probability to be proportional to the service rates of the storage nodes, i.e., $\pi_{ij}=k_{i}\frac{\mu_{j}}{\sum_{j}\mu_{j}}$. This achieves optimal load-balancing, because the chance of congestion is minimized in the storage system.


%we have the first 250 files access the first 4 servers with equal probabilities (=1), the last 250 files access the last 4 servers with equal probabilities (=1), whereas files 251 to 500 access the 12 servers with probabilities [0 17 17 17 18 3 0 0 0 0 0 0]/18, and files 501 to 750 access the servers with probabilities [0 0 0 0 16  46 52 52 25 25 0 0 ]/54. With this choice, the aggregate arrival rate at the first server is 3.33, at the last two servers is 5 and the rest 9 servers is 9.6296. 


%servers arrival rate at the first, 11th and 12th server can no longer be increased as each hosts only a single file.

%As a comparison, we have the initial choice of the access probabilities ${\bm \pi}$, and optimize over $t$. The other comparison is where we fix the ${\mathbf t}$ as in the initialization and optimize over the access probabilities ${\bm \pi}$.

We note that our proposed algorithm for jointly optimizing ${\bm \pi}$ and ${\mathbf t}$ provides significant improvement over simple heuristics such as Policies PEAP-OP, PEAP-RP, PPF-RP and PPF-OP, as weighted  latency tail probability reduces by an orders of magnitude. For example, our proposed Policy WLTP-OP decreases 99-percentile weighted latency (i.e., $x$ such that $\sum_i \omega_i\Pr(L_i \ge x)\le 0.01$) from above 220 seconds in the baseline policies to less than 40 seconds. Uniformly accessing servers and simple load-balancing are unable to optimize the request scheduler based on factors like chunk placement, request arrival rates, different latency weights, thus leading to much higher tail latency. We further notice that chunk placement optimization reduces  the latency tail probability further for all $x$.

%\input{lowx}

\begin{figure}
	\begin{center}
		\includegraphics[trim=.1in .1in .5in .1in, clip,width=0.80\textwidth]{convg}
		\caption{Convergence of Weighted Latency Tail Probability.}
		\label{convfig}
	\end{center}
\end{figure}


\noindent {\bf Convergence of the Proposed Algorithm: } We have shown that the proposed algorithm is guaranteed to converge. To illustrate its convergence speed, Figure \ref{convfig} shows the convergence of objective value vs. the number of iterations for different values of $x$ ranging from 50 to 190 seconds in increments of 20 seconds. For 1000 files and 12 storage nodes, we note that the weighted  latency tail probability shows convergence. In the rest of the results, 300 iterations are used and the results can only be better with higher number of iterations. 

%convergences very fast and within about 300 iterations to the optimal objective value, validating the efficiency of the proposed optimization algorithm.


\begin{figure}
	\begin{center}
		\includegraphics[trim=.0in .0in .3in .0in, clip,width=0.75\textwidth]{Lat_all}
		\caption{Weighted Latency Tail Probability for different file arrival rates. We vary
the arrival rate of file i from $0.2\times\lambda$ to $2\times\lambda$, where $\lambda$ is the base
arrival rate.}
		\label{arrfig}
	\end{center}
\end{figure}

\noindent {\bf Effect of Arrival Rates: } We next see the effect of varying request arrival rates on the weighted latency tail probability. We choose $x=50$ seconds. For $\lambda$ as the base arrival rates, we increase arrival rate of all files from $.2\lambda$ to $2\times\lambda$ and plot the weighted  latency tail probability in Figure~\ref{arrfig}. While latency tail probability increases as arrival rate goes up, our algorithm assigns differentiated latency for different files to maintain low weighted latency tail probability. We compare
our proposed algorithm with the different baseline policies and notice that the proposed algorithm outperforms all baseline strategies.

Since the latency tail probability is more significant at high arrival
rates, we observe significant improvement in latency tail
by about 43\% ( approximately 0.025 to about 0.22) at the highest
arrival rate in Figure 4 as compared to the optimized placement and
projected equal access policy. Our proposed policy always receives the minimum latency. Thus, efficiently reducing the latency of the high arrival rate files reduces the overall weighted latency tail probability.  

%We consider the arrival rates from $.6\lambda$ to $\lambda$ in Figure~\ref{arrfig}.  We see that the weighted tail latency increases with the arrival rate. Further, the third set of 250 files have a much higher weight and thus the algorithm tries to decrease the latencies of this set of files significantly at the expense of the other files.

\begin{figure}
	\begin{center}
		\includegraphics[trim=.0in .1in 5.8in .0in,clip,width=0.45\textwidth]{numberOfFiles}
		\caption{Weighted Latency Tail Probability for different number of files.}
		\label{filesfig}
	\end{center}
\end{figure}


\noindent {\bf Effect of Number of files: } Figure \ref{filesfig} demonstrates the impact of varying the number of video files from 200 files to 1200 files on the weighted latency tail probability. Weighted latency tail  probabilities increases with the number of files, which brings in more workload (i.e., higher arrival rates). Our optimization algorithm optimizes new files along with existing ones to keep overall latency tail probability at a very low level. We note that the proposed optimization strategy effectively reduces the tail probability and outperforms the considered baseline strategies. Thus, joint optimization over all three variables $\boldsymbol{\mathcal{S}}$,$\boldsymbol{\pi}$ , and $\boldsymbol{t}$ helps reduce the tail probability dramatically .


==> lowx.tex <==
\begin{figure}
	\begin{center}
		\includegraphics[trim=.2in 2.6in .9in 2.9in, clip,width=0.45\textwidth]{zoom_lowx.pdf}
		\caption{Weighted  Latency Tail Probability vs $x$ (in seconds).}
		\label{tailfig2}
	\end{center}
\end{figure}

Figure \ref{tailfig2} further gives a zoomed-in plot for the weighted tail latency as a function of $x$ when $x$ varies from 10 to 40.
